SPARC: Score Prompting and Adaptive Fusion for Zero-Shot Multi-Label Recognition in Vision-Language Models

Zero-shot multi-label recognition (MLR) with Vision-Language Models (VLMs) faces significant challenges without training data, model tuning, or architectural modifications. Existing approaches require prompt tuning or architectural adaptations, limiting zero-shot applicability. Our work proposes a novel solution treating VLMs as black boxes, leveraging scores without training data or ground truth. Using large language model insights on object co-occurrence, we introduce compound prompts grounded in realistic object combinations. Analysis of these prompt scores reveals VLM biases and ``AND''/``OR'' signal ambiguities, notably that maximum compound scores are surprisingly suboptimal compared to second-highest scores. We address these through a debiasing and score-fusion algorithm that corrects image bias and clarifies VLM response behaviors. Our method enhances other zero-shot approaches, consistently improving their results. Experiments show superior mean Average Precision (mAP) compared to methods requiring training data, achieved through refined object ranking for robust zero-shot MLR.

==> sec/tables/competition_table_TagCLIP_CustomResolution.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{llcc|c}
\toprule
    &             &       COCO ViT-B/16 &       VOC ViT-B/16 &            Avg \\
\midrule
 & TagCLIP &           70.9 &           91.7 &           81.3 \\
    & $+$Ours &           \textbf{73.8} &           \textbf{92.0} &  \textbf{82.9} \\
\bottomrule
\end{tabular}
\vspace{-2pt}
\caption{Rerun of Tab.3 with matching preproc/res settings}
\label{tab:CompetitionTagCLIPlogYESrowcalibbaseNOCustomResolution}
\end{table}


==> sec/tables/main_tables_tersified_USE_DPT.tex <==
\begin{table}[ht]
\centering
\scalebox{0.95}{
\begin{tabular}{llccccc}
\toprule
                         &                   & \makecell{RN50 \\ x64} & \makecell{RN50 \\ x16} & \makecell{RN50 \\ x4} & \makecell{RN \\ 101} & \makecell{RN \\ 50} \\
\midrule
\multirow{2}{*}{COCO}    & CLIP-DPT & 70.5 & 64.2 & 64.2 & 59.7 & 57.1 \\
                         & Ours-DPT & \textbf{77.8} &  \textbf{73.9} &  \textbf{72.7} &  \textbf{69.8} &  \textbf{68.4} \\
\midrule
\multirow{2}{*}{VOC}     & CLIP-DPT & 86.6 & 82.4 & 86.1 & 83.5 & 82.6 \\
                         & Ours-DPT & \textbf{91.1} & \textbf{89.8} & \textbf{88.5} & \textbf{88.5} & \textbf{89.9} \\
\midrule
\multirow{2}{*}{NUS}    & CLIP-DPT & 39.8 & 37.8 & 39.3 & 38.4 & 38.1 \\
                         & Ours-DPT & \textbf{43.5} & \textbf{45.5} & \textbf{42.7} & \textbf{42.6} & \textbf{44.5} \\
\bottomrule
\end{tabular}
}
\vspace{-7pt}
\caption{Comparing SPARC with local method CLIP-DPT [5].}
\label{tab:MainTableThreeDatasetsDPT}
\end{table}

